The Good, The Efficient and the Inductive Biases: Exploring Efficiency in Deep Learning Through the Use of Inductive Biases

The emergence of Deep Learning has marked a profound shift in machine learning, driven by numerous breakthroughs achieved in recent years. However, as Deep Learning becomes increasingly present in everyday tools and applications, there is a growing need to address unresolved challenges related to its efficiency and sustainability. This dissertation delves into the role of inductive biases -- particularly, continuous modeling and symmetry preservation -- as strategies to enhance the efficiency of Deep Learning. It is structured in two main parts. The first part investigates continuous modeling as a tool to improve the efficiency of Deep Learning algorithms. Continuous modeling involves the idea of parameterizing neural operations in a continuous space. The research presented here demonstrates substantial benefits for the (i) computational efficiency -- in time and memory, (ii) the parameter efficiency, and (iii) design efficiency -- the complexity of designing neural architectures for new datasets and tasks. The second focuses on the role of symmetry preservation on Deep Learning efficiency. Symmetry preservation involves designing neural operations that align with the inherent symmetries of data. The research presented in this part highlights significant gains both in data and parameter efficiency through the use of symmetry preservation. However, it also acknowledges a resulting trade-off of increased computational costs. The dissertation concludes with a critical evaluation of these findings, openly discussing their limitations and proposing strategies to address them, informed by literature and the author insights. It ends by identifying promising future research avenues in the exploration of inductive biases for efficiency, and their wider implications for Deep Learning.

==> backmatter/colophon.tex <==

\cleartoleftpage
\par\vbox{}\null\vfill\nopagebreak
%\vspace*{350pt}

%\begin{center}
%\footnotesize
\small
\noindent
\parbox{105mm}{\textsc{This thesis was typeset} using \LaTeX. The template used by this thesis was adapted from templates by John \mbox{Papandriopoulos} (\url{http://jpap.org/projects.html}) and Jordan Suchow (\url{https://github.com/suchow/Dissertate}). A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}} license, and can be found online at \href{https://github.com/XXXX} or from its lead author, Maoyuan Liu, at \mbox{\href{mailto:contact@mao.id.au}{contact@mao.id.au}}.}
%\end{center}


==> chapters/discussion.tex <==
% path to figures directory
\graphicspath{{figures/0-meta/}}

%=========================================================================

\chapter{Discussion} \label{chapter:discussion}

==> frontmatter/abstract.tex <==
\begin{abstract}%

{\scshape TODO}

\end{abstract}


==> frontmatter/dedication.tex <==
\begin{dedication}
    To my loving family, 
\end{dedication}


==> frontmatter/samenvatting.tex <==
\begin{samenvatting}%

{\scshape TODO}

\end{samenvatting}


==> tables/appx-classification-1d.tex <==
\begin{table}
\centering
\vskip -2mm
\caption{Test accuracy on sMNIST, pMNIST, sCIFAR10 and npCIFAR10. \todo{Conclusions?}}
\label{tab:full-smnist}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{sMNIST} & \sc{pMNIST} & \sc{sCIFAR10} & \sc{npCIFAR10} \\
 \midrule
 DilRNN \citep{chang2017dilated} & 44\sc{k} & 98.0 & 96.1 & - & -\\
  IndRNN \citep{li2018independently} & 83\sc{k} & 99.0 & 96.0& - & - \\
  %LSTM \citep{bai2018empirical} &70\sc{k}& 87.2 & 85.7  & - \\
 %GRU \citep{bai2018empirical} &70\sc{k}&   96.2 & 87.3  & - \\
   TCN \citep{bai2018empirical} &70\sc{k}& 99.0 & 97.2  & - & - \\
  r-LSTM \citep{trinh2018learning} & 0.5\sc{m} & 98.4 & 95.2 & 72.2 & -\\
 Self-Att. \citep{trinh2018learning} &0.5\sc{m} & 98.9 & 97.9 & 62.2 & -\\
 TrellisNet \citep{bai2018trellis}& 8\sc{m} & 99.20 & 98.13 & 73.42 & - \\
 URLSTM \citep{gu2020improving} & - & 99.28 & 96.96 & 71.00 & - \\
  URGRU + Zoneout \citep{gu2020improving} & - & 99.27 & 96.51 & \textbf{74.40} & - \\
  HiPPO \citep{gu2020hippo} & 0.5\sc{m} & - & \textbf{98.30} & - & - \\
  Lipschitz RNN \citep{erichson2020lipschitz} & 158\sc{k} & 99.4 & 97.3 & 64.2 & 59.0 \\
  coRNN \citep{rusch2020coupled} & 134\sc{k} & \textbf{99.4} & 97.3 & - & 59.0 \\
  UnICORNN \citep{rusch2021unicornn} & 135\sc{k} & - & 98.4 & - & \textbf{62.4} \\
  pLMU \citep{chilkuri2021parallelizing} & 165\sc{k} & - & 98.49 & - & -\\
\midrule
CKCNN-2 & 98\sc{k} & 99.31 & 98.00 & 62.25 & 60.5\\
CKCNN-2-Big & 1\sc{m} & 99.32 & 98.54 & 63.74 & 62.2 \\
CKTCN$_{\text{\sc{Fourier}}}$-2 & \todo{...\sc{m}} & 99.44 & 98.40 & 68.28 & 66.26 \\
CKTCN$_{\text{\sc{Gabor}}}$-2 & \todo{...\sc{m}} & 99.52 & 98.38 & 69.26 & 67.52 \\
CKTCN$_{\text{\sc{MAGNet}}}$-2 & 105\sc{k} & \textbf{99.55} &\textbf{ 98.57} & \textbf{74.58} & \textbf{67.37} \\
\midrule
FlexTCN-2 & 108\sc{k} & \textbf{99.60} & \textbf{98.61} & \textbf{78.99} &  \textbf{67.11}\\
FlexTCN-4 &  241\sc{k} & \textbf{99.60} & \textbf{98.72} & \textbf{80.26} & \textbf{67.42}\\
FlexTCN-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\midrule
FlexTCN$_{\text{SIREN}}$-6 & \todo{...\sc{m}} & 99.03 & 95.36 & 69.24 & 57.27 \\
FlexTCN$_{\text{Fourier}}$-6 & \todo{...\sc{m}} & 99.49 & 97.97 & 74.79 & 67.35 \\
FlexTCN$_{\text{Gabor}}$-6 & \todo{...\sc{m}} &  99.50 & 98.37 & 78.36 & 67.56 \\
FlexTCN$_{\text{MAGNet}}$-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\bottomrule
\end{tabular}}
\end{small}
\end{table}

==> tables/classification-1d.tex <==
\begin{table}
\centering
\vskip -2mm
\caption{Test accuracy on sMNIST, pMNIST, sCIFAR10 and npCIFAR10. \todo{Conclusions.} \todo{Select models \& ablations to keep.} Tab.~\ref{tab:full-smnist} shows more results, including more baselines and ablations.}
\label{tab:smnist}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{sMNIST} & \sc{pMNIST} & \sc{sCIFAR10} & \sc{npCIFAR10} \\
 \midrule
 DilRNN & 44\sc{k} & 98.0 & 96.1 & - & -\\
  IndRNN & 83\sc{k} & 99.0 & 96.0& - & - \\
  %LSTM \citep{bai2018empirical} &70\sc{k}& 87.2 & 85.7  & - \\
 %GRU \citep{bai2018empirical} &70\sc{k}&   96.2 & 87.3  & - \\
   TCN &70\sc{k}& 99.0 & 97.2  & - & - \\
  r-LSTM & 0.5\sc{m} & 98.4 & 95.2 & 72.2 & -\\
 Self-Att. &0.5\sc{m} & 98.9 & 97.9 & 62.2 & -\\
 TrellisNet & 8\sc{m} & 99.20 & 98.13 & 73.42 & - \\
 URLSTM & - & 99.28 & 96.96 & 71.00 & - \\
  URGRU + Zoneout  & - & 99.27 & 96.51 & 74.40 & - \\
  HiPPO & 0.5\sc{m} & - & 98.30 & - & - \\
  Lipschitz RNN & 158\sc{k} & 99.4 & 97.3 & 64.2 & 59.0 \\
  coRNN & 134\sc{k} & 99.4 & 97.3 & - & 59.0 \\
  UnICORNN & 135\sc{k} & - & 98.4 & - & 62.4 \\
  pLMU  & 165\sc{k} & - & 98.49 & - & -\\
\midrule
CKCNN-2 & 98\sc{k} & 99.31 & 98.00 & 62.25 & 60.5\\
CKCNN-2-Big & 1\sc{m} & 99.32 & 98.54 & 63.74 & 62.2 \\
CKTCN$_{\text{\sc{Fourier}}}$-2 & & 99.44 & 98.40 & 68.28 & 66.26 \\
CKTCN$_{\text{\sc{Gabor}}}$-2 & & 99.52 & 98.38 & 69.26 & 67.52 \\
CKTCN$_{\text{\sc{MAGNet}}}$-2 & 105\sc{k} & 99.55 & 98.57 & 74.58 & 67.37 \\
\midrule
FlexTCN-2 & 108\sc{k} & 99.60 & 98.61 & 78.99 & 67.11\\
FlexTCN-4 &  241\sc{k} & 99.60 & \textbf{98.72} & 80.26 & 67.42\\
FlexTCN-6 & 375\sc{k} & \textbf{99.62} &  98.63 & \textbf{80.82} & \textbf{69.87} \\
\midrule
\midrule
FlexTCN$_{\text{SIREN}}$-6 &  & 99.03 & 95.36 & 69.24 & 57.27 \\
FlexTCN$_{\text{Fourier}}$-6 & & 99.49 & 97.97 & 74.79 & 67.35 \\
FlexTCN$_{\text{Gabor}}$-6 & &  99.50 & 98.37 & 78.36 & 67.56 \\
FlexTCN$_{\text{MAGNet}}$-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\bottomrule
\end{tabular}}
\end{small}
\end{table}

% DilRNN \citep{chang2017dilated}, 
% IndRNN \citep{li2018independently}, 
% TCN \citep{bai2018empirical}, 
% r-LSTM \citep{trinh2018learning}, 
% Self-Att. \citep{trinh2018learning}, 
% TrellisNet \citep{bai2018trellis}, 
% URLSTM \citep{gu2020improving}, 
% URGRU + Zoneout \citep{gu2020improving}, 
% HiPPO \citep{gu2020hippo}, 
% Lipschitz RNN \citep{erichson2020lipschitz}, 
% coRNN \citep{rusch2020coupled}, 
% UnICORNN \citep{rusch2021unicornn} and
% pLMU \citep{chilkuri2021parallelizing}.

==> tables/classification-cifar10.tex <==
\begin{table}
% \begin{wraptable}{r}{0.45\textwidth}
\vspace{-0mm}
\centering
\caption{Results on CIFAR-10. FlexNet is competitive with CIFARResNets and other learnable kernel size works. The FlexConv mask and MAGNet both improve over the baseline CKConv methods. We report results over three runs per setting. Time is reported as seconds per epoch of a converged model. Tab.~\ref{tab:full-cifar-10} shows more results, including more ablations. *Results are taken from the respective original works instead of reproduced. \!\dagger Results are from single run.}
\label{tab:cifar-10}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \sc{CIFAR-10} & \multirow{2}{*}{\sc{Time}} \\
    & & \sc{Acc.} & \\ \midrule
    CIFARResNet-44 & 0.66\sc{m} & 92.9*\!\dagger & - \\ \midrule
    DCN-$\sigma^{ji}$ & 0.47\sc{m} & 89.7 $\pm$ 0.3* & - \\
    N-Jet-CIFARResNet32 & 0.52\sc{m} & 92.3 $\pm$ 0.3* & - \\
    N-Jet-ALLCNN & 1.07\sc{m} & 92.5 $\pm$ 0.1* & - \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 89.5 $\pm$ 0.3 & 41s   \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 78.0 $\pm$ 0.3 & 242s  \\
    FlexNet-7 w/ N-Jet & 0.70\sc{m} & 91.7 $\pm$ 0.1 & 409s  \\ \midrule
    % \midrule
    CKCNN-7 & 0.63\sc{m} & 71.7* & 266s \\ % 71.70
    CKCNN$_{\text{Gabor}}$-7 & 0.67\sc{m} & 87.6* & \todo{69s} \\ % 87.65
    CKCNN$_{\text{MAGNet}}$-7 & 0.67\sc{m} &  85.9* & 299s \\ % 85.91
    \midrule
    FlexNet$_{\text{SIREN}}$-7 & 0.63\sc{m} & 88.9* & 105s \\ % 88.88
    FlexNet$_{\text{Gabor}}$-7 & 0.67\sc{m} & 92.0* & 178s \\ % 91.99
    \midrule
    FlexNet-7 & 0.67\sc{m} & 92.2 $\pm$ 0.1 & 166s \\
 \bottomrule
\end{tabular}}
% \end{sc}
% \end{small}
\end{center}
\vspace{-7mm}
\end{table}
% \end{wraptable}

==> tables/classification-sequences.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\vspace{-5mm}
\vskip -2mm
\caption{Test accuracy on Character Trajectory, Speech Commands, Speech Commands Raw. \todo{Conclusions.}}
\label{tab:time-series}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{CT} & \sc{SC} & \sc{SC\_raw} \\
\midrule
GRU-ODE & 89\sc{k} & 96.2 & 44.8 & $\sim$10.0 \\
GRU-$\Delta t$ & 89\sc{k} & 97.8 & 20.0 & $\sim$10.0 \\
GRU-D & 89\sc{k} & 95.9 & 23.9 & $\sim$10.0 \\
ODE-RNN & 89\sc{k} & 97.1 & 93.2 & $\sim$10.0 \\
NCDE  & 89\sc{k} & 98.8 & 88.5 & $\sim$10.0 \\
\midrule
CKCNN & 100\sc{k} &\textbf{ 99.53 }& 95.27 & 71.66 \\
CKTCN$_{\text{Fourier}}$ & & - & 95.65 & 74.90 \\
CKTCN$_{\text{Gabor}}$ &  & - & 96.66 &  78.10 \\
CKTCN$_{\text{MAGNet}}$ & 105\sc{k} &  \textbf{99.53} & \textbf{97.01} & \textbf{80.69} \\
\midrule
FlexTCN-2 & 105\sc{sk} & \textbf{99.53} & \textbf{97.10} & \textbf{88.03}  \\
FlexTCN-4 & 239\sc{k} & \textbf{99.53} & \textbf{97.73} & \textbf{90.45}   \\
FlexTCN-6 & 373\sc{k} & \textbf{99.53} & \textbf{97.67} & \textbf{91.73} \\
\midrule
FlexTCN$_{\text{SIREN}}$-6 &  & - & 95.83 & \\
FlexTCN$_{\text{Fourier}}$-6 & & - & 97.62 &  \\
FlexTCN$_{\text{Gabor}}$-6 & & - & 97.35 & \\
FlexTCN$_{\text{MAGNet}}$-6 & 373\sc{k} & - & \textbf{97.67} & \textbf{91.73} \\
\bottomrule
\end{tabular}}
\end{small}
\vspace{5mm}
\end{wraptable}

==> tables/crossres-cifar10.tex <==
\begin{table}

\begin{minipage}{0.50\textwidth}
\vspace{8mm}
\centering
\caption{Results for alias-free FlexNets on \todo{CIFAR-10}.
% FlexNets reduce the accuracy gap at upscaling more than all other methods. We train each model for 100 epochs at resolution $16 \times 16$, then evaluate it at resolution $32 \times 32$. We report results over three runs per setting.
}
\label{tab:crossres}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \multicolumn{2}{c}{\sc{CIFAR-10 Acc.}} \\
    & & 16 px & $\Delta_{16 \textrm{px}}$ 32 px \\ \midrule % & fine-tuned \\ \midrule
    CIFARResNet-44 & 0.66\sc{m} & 85.8 $\pm$ 0.2 & -31.6 $\pm$ 1.3 \\ \midrule
    % 85.4 $\pm$ 0.3 & -31.2 $\pm$ 2.8 \\ \midrule % & 92.6 $\pm$ 0.2 \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 85.3 $\pm$ 0.2 & -21.2 $\pm$ 1.0 \\ % & \textbf{90.1} $\pm$ 0.1  \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 67.7 $\pm$ 0.6 & -57.1 $\pm$ 1.6 \\ % & 79.2 $\pm$ 0.4  \\
    FlexNet-7 w/ N-Jets & 0.70\sc{m} & \textbf{86.4} $\pm$ 0.2 & -5.5 $\pm$ 1.3 \\ \midrule % & 89.5 $\pm$ 0.1  \\ \midrule
    CKCNN-7$_{\textrm{SIREN}}$ & 0.63\sc{m} & 45.9 $\pm$ 1.0 & -15.8 $\pm$ 1.2 \\
    FlexNet-7$_{\textrm{SIREN}}$ & 0.63\sc{m} & 70.4 $\pm$ 0.8 & -50.0 $\pm$ 16.9 \\ \midrule
    FlexNet-7 w/o reg. & 0.67\sc{m} & \textbf{86.4} $\pm$ 0.4 & -34.4 $\pm$ 14.3 \\ \midrule % & 88.8 $\pm$ 0.6 \\ \midrule
    FlexNet-7 w/ reg. $f^+_{\textrm{MAGNet}}$ & 0.67\sc{m} & \textbf{86.5} $\pm$ 0.1 & -3.8 $\pm$ 2.0 \\ % & 89.0 $\pm$ 0.3  \\
    FlexNet-7 w/ reg. $f^+_{\textrm{FlexConv}}$ & 0.67\sc{m} & 85.1 $\pm$ 0.3 & \textbf{-3.3} $\pm$ 0.3 \\ % & 87.6 $\pm$ 0.2 \\
 \bottomrule
\end{tabular}}
\end{center}
% \vspace{-5mm}
\end{minipage}\hspace{5mm}
\end{table}
